Beating stellar systematic error floors using transit-based densities

It has long been understood that the light curve of a transiting planet constrains the density of its host star. That fact is routinely used to improve measurements of the stellar surface gravity and has been argued to be an independent check on the stellar mass. Here we show how the stellar density can also dramatically improve the precision of the radius and effective temperature of the star. This additional constraint is especially significant when we properly account for the 4.2% radius and 2.0% temperature systematic errors inherited from photometric zero-points, model atmospheres, interferometric calibration, and extinction. In the typical case, we can constrain stellar radii to 3% and temperatures to 1.75% with our evolutionary-model-based technique. In the best real-world cases, we can infer radii to 1.6% and temperatures to 1.1% -- well below the systematic measurement floors -- which can improve the precision in the planetary parameters by a factor of two. We explain in detail the mechanism that makes it possible and show a demonstration of the technique for a near-ideal system, WASP-4. We also show that both the statistical and systematic uncertainties in the parallax from Gaia DR3 are often a significant component of the uncertainty in $L_*$ and must be treated carefully. Taking advantage of our technique requires simultaneous models of the stellar evolution, bolometric flux (e.g., a stellar spectral energy distribution), and the planetary transit, while accounting for the systematic errors in each, as is done in EXOFASTv2.

==> tab3.tex <==
\begin{turnpage}

\begin{table*}
	\centering
	\caption{Median values and 68\% confidence interval for the WASP-4 host star}
	\label{tab:wasp4}
	\begin{tabular}{llcccccccc}
	\toprule	\colhead{~~~Parameter} & \colhead{Units} & \colhead{None} & \colhead{MIST} & \colhead{SED} & \colhead{MIST+SED} & \colhead{Transit} & \colhead{Transit+SED} & \colhead{MIST+Transit} & \colhead{MIST+Transit+SED} \\
	\toprule
 ~~~~$M_*$\dotfill&Mass (\msun)\dotfill &$0.88^{+0.15}_{-0.13}$&$0.879^{+0.056}_{-0.048}$&$0.88^{+0.15}_{-0.13}$&$0.895^{+0.052}_{-0.046}$&$0.91^{+0.13}_{-0.14}$&$0.88^{+0.13}_{-0.11}$&$0.890^{+0.070}_{-0.057}$&$0.886^{+0.046}_{-0.040}$\\
~~~~$R_*$\dotfill&Radius (\rsun)\dotfill &$0.900^{+0.046}_{-0.047}$&$0.890^{+0.049}_{-0.041}$&$0.890^{+0.044}_{-0.038}$&$0.886^{+0.035}_{-0.032}$&$0.903^{+0.043}_{-0.048}$&$0.893^{+0.041}_{-0.038}$&$0.898^{+0.023}_{-0.020}$&$0.896^{+0.015}_{-0.014}$\\
~~~~$L_*$\dotfill&Luminosity (\lsun)\dotfill &$0.631^{+0.12}_{-0.097}$&$0.63^{+0.12}_{-0.10}$&$0.624^{+0.029}_{-0.028}$&$0.624^{+0.030}_{-0.027}$&$0.631^{+0.12}_{-0.097}$&$0.624^{+0.028}_{-0.026}$&$0.65\pm0.11$&$0.625^{+0.028}_{-0.026}$\\
~~~~$\rho_*$\dotfill&Density (cgs)\dotfill &$1.70^{+0.38}_{-0.31}$&$1.76^{+0.24}_{-0.23}$&$1.74^{+0.37}_{-0.30}$&$1.82^{+0.24}_{-0.22}$&$1.737^{+0.019}_{-0.025}$&$1.737^{+0.019}_{-0.025}$&$1.738^{+0.018}_{-0.025}$&$1.738^{+0.018}_{-0.024}$\\
~~~~$\log{g}$\dotfill&Surface gravity (cgs)\dotfill &$4.473\pm0.074$&$4.483^{+0.039}_{-0.042}$&$4.480^{+0.074}_{-0.073}$&$4.495^{+0.041}_{-0.042}$&$4.484^{+0.020}_{-0.024}$&$4.479^{+0.020}_{-0.019}$&$4.481^{+0.011}_{-0.010}$&$4.4809^{+0.0080}_{-0.0078}$\\
~~~~$T_{\rm eff}$\dotfill&Effective Temperature (K)\dotfill &$5430^{+210}_{-200}$&$5440^{+180}_{-190}$&$5440\pm120$&$5450\pm100$&$5420\pm210$&$5430\pm120$&$5470^{+180}_{-200}$&$5419^{+65}_{-63}$\\
~~~~$[{\rm Fe/H}]$\dotfill&Metallicity (dex)\dotfill &$-0.031\pm0.087$&$-0.025\pm0.089$&$0.011^{+0.085}_{-0.083}$&$0.012^{+0.082}_{-0.080}$&$-0.031^{+0.091}_{-0.090}$&$0.013^{+0.082}_{-0.079}$&$-0.021^{+0.089}_{-0.088}$&$0.015^{+0.082}_{-0.078}$\\
~~~~$[{\rm Fe/H}]_{0}$\dotfill&Initial Metallicity$^{2}$ \dotfill &--&$-0.00\pm0.11$&--&$0.03\pm0.10$&--&--&$0.00\pm0.11$&$0.033^{+0.10}_{-0.099}$\\
~~~~$Age$\dotfill&Age (Gyr)\dotfill &--&$7.0^{+4.4}_{-3.7}$&--&$6.2^{+4.7}_{-3.9}$&--&--&$6.6^{+4.4}_{-4.0}$&$7.3^{+3.7}_{-3.8}$\\
~~~~$EEP$\dotfill&Equal Evolutionary Phase$^{3}$ \dotfill &--&$351^{+37}_{-18}$&--&$350^{+37}_{-27}$&--&--&$351^{+33}_{-23}$&$356^{+32}_{-22}$\\
~~~~$R_{*,SED}$\dotfill&Radius$^{1}$ (\rsun)\dotfill &--&--&$0.882^{+0.017}_{-0.016}$&$0.882^{+0.017}_{-0.016}$&--&$0.882\pm0.016$&--&$0.883^{+0.016}_{-0.015}$\\
~~~~$F_{Bol}$\dotfill&Bolometric Flux (cgs)\dotfill &--&--&$0.0000000002867^{+0.0000000000098}_{-0.0000000000088}$&$0.0000000002870^{+0.0000000000095}_{-0.0000000000088}$&--&$0.0000000002866^{+0.0000000000092}_{-0.0000000000082}$&--&$0.0000000002867^{+0.0000000000088}_{-0.0000000000082}$\\
~~~~$T_{\rm eff,SED}$\dotfill&Effective Temperature$^{1}$ (K)\dotfill &--&--&$5461^{+34}_{-31}$&$5462^{+33}_{-30}$&--&$5461^{+31}_{-29}$&--&$5460^{+30}_{-29}$\\
~~~~$[{\rm Fe/H}]_{SED}$\dotfill&Metallicity (dex)\dotfill &--&--&$0.038^{+0.11}_{-0.092}$&$0.042^{+0.11}_{-0.096}$&--&$0.043^{+0.10}_{-0.089}$&--&$0.043^{+0.11}_{-0.087}$\\
~~~~$A_V$\dotfill&V-band extinction (mag)\dotfill &--&--&$0.022^{+0.014}_{-0.015}$&$0.023^{+0.014}_{-0.015}$&--&$0.023^{+0.014}_{-0.015}$&--&$0.023^{+0.014}_{-0.015}$\\
~~~~$\sigma_{SED}$\dotfill&SED photometry error scaling \dotfill &--&--&$1.02^{+0.41}_{-0.24}$&$1.01^{+0.40}_{-0.24}$&--&$0.98^{+0.34}_{-0.22}$&--&$0.97^{+0.33}_{-0.21}$\\
~~~~$\varpi$\dotfill&Parallax (mas)\dotfill &--&--&$3.791\pm0.061$&$3.791\pm0.061$&--&$3.791^{+0.059}_{-0.060}$&--&$3.789^{+0.059}_{-0.060}$\\
~~~~$d$\dotfill&Distance (pc)\dotfill &--&--&$263.8^{+4.3}_{-4.2}$&$263.8^{+4.3}_{-4.2}$&--&$263.8^{+4.2}_{-4.1}$&--&$264.0^{+4.2}_{-4.1}$\\
		\hline
	\end{tabular}
\tablenotetext{}{See Table 3 in \citet{Eastman:2019} for a detailed description of all parameters\hfill\hfill}
\tablenotetext{1}{This value ignores the systematic error and is for reference only}
\tablenotetext{2}{The metallicity of the star at birth}
\tablenotetext{3}{Corresponds to static points in a star's evolutionary history. See \S2 in \citet{Dotter:2016}.}

\end{table*}
	
\end{turnpage}

==> tab4.tex <==
\newcommand{\rptabfourone}{$1.348^{+0.064}_{-0.071}$}
\newcommand{\mptabfourone}{$1.22\pm0.13$}
\newcommand{\atabfourone}{$0.0230^{+0.0011}_{-0.0012}$}
\newcommand{\teqtabfourone}{$1638^{+64}_{-63}$}
\newcommand{\tcirctabfourone}{$0.00277^{+0.00021}_{-0.00020}$}
\newcommand{\rhoptabfourone}{$0.620^{+0.045}_{-0.042}$}
\newcommand{\loggptabfourone}{$3.222^{+0.022}_{-0.023}$}
\newcommand{\favetabfourone}{$1.64^{+0.27}_{-0.24}$}
\newcommand{\msinitabfourone}{$1.22\pm0.13$}
\newcommand{\periodtabfourone}{$1.338231512\pm0.000000019$}
\newcommand{\tctabfourone}{$2454697.797524\pm0.000024$}
\newcommand{\tttabfourone}{$2454697.797524\pm0.000024$}
\newcommand{\tstabfourone}{$2454698.466639\pm0.000024$}
\newcommand{\tzerotabfourone}{$2455337.472187\pm0.000022$}
\newcommand{\itabfourone}{$88.87^{+0.67}_{-0.51}$}
\newcommand{\btabfourone}{$0.108^{+0.048}_{-0.064}$}
\newcommand{\ktabfourone}{$240\pm12$}
\newcommand{\ptabfourone}{$0.15348^{+0.00047}_{-0.00039}$}
\newcommand{\artabfourone}{$5.481^{+0.020}_{-0.026}$}
\newcommand{\deltatabfourone}{$0.02356^{+0.00014}_{-0.00012}$}
\newcommand{\deltartabfourone}{$0.03042^{+0.00086}_{-0.00081}$}
\newcommand{\deltaztabfourone}{$0.02781^{+0.00049}_{-0.00046}$}
\newcommand{\deltattabfourone}{$0.02867^{+0.00076}_{-0.00072}$}
\newcommand{\tautabfourone}{$0.01220^{+0.00017}_{-0.00013}$}
\newcommand{\tonefourtabfourone}{$0.08992\pm0.00014$}
\newcommand{\tfwhmtabfourone}{$0.07770^{+0.00017}_{-0.00018}$}
\newcommand{\ruonetabfourone}{$0.460\pm0.041$}
\newcommand{\rutwotabfourone}{$0.152^{+0.075}_{-0.076}$}
\newcommand{\zuonetabfourone}{$0.312^{+0.025}_{-0.024}$}
\newcommand{\zutwotabfourone}{$0.219^{+0.055}_{-0.057}$}
\newcommand{\tuonetabfourone}{$0.364^{+0.041}_{-0.040}$}
\newcommand{\tutwotabfourone}{$0.141^{+0.075}_{-0.076}$}
\newcommand{\rptabfourtwo}{$1.335^{+0.062}_{-0.058}$}
\newcommand{\mptabfourtwo}{$1.20^{+0.13}_{-0.11}$}
\newcommand{\atabfourtwo}{$0.02277^{+0.0010}_{-0.00099}$}
\newcommand{\teqtabfourtwo}{$1639^{+35}_{-36}$}
\newcommand{\tcirctabfourtwo}{$0.00279\pm0.00021$}
\newcommand{\rhoptabfourtwo}{$0.624^{+0.042}_{-0.041}$}
\newcommand{\loggptabfourtwo}{$3.222^{+0.021}_{-0.023}$}
\newcommand{\favetabfourtwo}{$1.64^{+0.15}_{-0.14}$}
\newcommand{\msinitabfourtwo}{$1.20^{+0.13}_{-0.11}$}
\newcommand{\periodtabfourtwo}{$1.338231512\pm0.000000019$}
\newcommand{\tctabfourtwo}{$2454697.797525\pm0.000024$}
\newcommand{\tttabfourtwo}{$2454697.797525\pm0.000024$}
\newcommand{\tstabfourtwo}{$2454698.466641\pm0.000024$}
\newcommand{\tzerotabfourtwo}{$2455348.178040\pm0.000022$}
\newcommand{\itabfourtwo}{$88.87^{+0.67}_{-0.51}$}
\newcommand{\btabfourtwo}{$0.109^{+0.048}_{-0.064}$}
\newcommand{\ktabfourtwo}{$240\pm12$}
\newcommand{\ptabfourtwo}{$0.15349^{+0.00047}_{-0.00040}$}
\newcommand{\artabfourtwo}{$5.481^{+0.020}_{-0.026}$}
\newcommand{\deltatabfourtwo}{$0.02356^{+0.00014}_{-0.00012}$}
\newcommand{\deltartabfourtwo}{$0.03044^{+0.00086}_{-0.00082}$}
\newcommand{\deltaztabfourtwo}{$0.02782^{+0.00049}_{-0.00047}$}
\newcommand{\deltattabfourtwo}{$0.02869^{+0.00075}_{-0.00071}$}
\newcommand{\tautabfourtwo}{$0.01220^{+0.00017}_{-0.00013}$}
\newcommand{\tonefourtabfourtwo}{$0.08992\pm0.00014$}
\newcommand{\tfwhmtabfourtwo}{$0.07770^{+0.00017}_{-0.00018}$}
\newcommand{\ruonetabfourtwo}{$0.461^{+0.041}_{-0.042}$}
\newcommand{\rutwotabfourtwo}{$0.151\pm0.076$}
\newcommand{\zuonetabfourtwo}{$0.313\pm0.025$}
\newcommand{\zutwotabfourtwo}{$0.218^{+0.056}_{-0.057}$}
\newcommand{\tuonetabfourtwo}{$0.365\pm0.040$}
\newcommand{\tutwotabfourtwo}{$0.139^{+0.074}_{-0.075}$}
\newcommand{\rptabfourthree}{$1.341^{+0.035}_{-0.030}$}
\newcommand{\mptabfourthree}{$1.210^{+0.086}_{-0.081}$}
\newcommand{\atabfourthree}{$0.02287^{+0.00060}_{-0.00052}$}
\newcommand{\teqtabfourthree}{$1651^{+54}_{-61}$}
\newcommand{\tcirctabfourthree}{$0.00278\pm0.00019$}
\newcommand{\rhoptabfourthree}{$0.621\pm0.036$}
\newcommand{\loggptabfourthree}{$3.222^{+0.021}_{-0.023}$}
\newcommand{\favetabfourthree}{$1.69^{+0.23}_{-0.24}$}
\newcommand{\msinitabfourthree}{$1.210^{+0.086}_{-0.081}$}
\newcommand{\periodtabfourthree}{$1.338231512\pm0.000000019$}
\newcommand{\tctabfourthree}{$2454697.797524^{+0.000024}_{-0.000023}$}
\newcommand{\tttabfourthree}{$2454697.797524^{+0.000024}_{-0.000023}$}
\newcommand{\tstabfourthree}{$2454698.466640^{+0.000024}_{-0.000023}$}
\newcommand{\tzerotabfourthree}{$2455336.133956\pm0.000022$}
\newcommand{\itabfourthree}{$88.89^{+0.66}_{-0.52}$}
\newcommand{\btabfourthree}{$0.106^{+0.049}_{-0.063}$}
\newcommand{\ktabfourthree}{$240\pm12$}
\newcommand{\ptabfourthree}{$0.15348^{+0.00047}_{-0.00039}$}
\newcommand{\artabfourthree}{$5.482^{+0.019}_{-0.026}$}
\newcommand{\deltatabfourthree}{$0.02355^{+0.00015}_{-0.00012}$}
\newcommand{\deltartabfourthree}{$0.03043^{+0.00086}_{-0.00081}$}
\newcommand{\deltaztabfourthree}{$0.02782^{+0.00050}_{-0.00047}$}
\newcommand{\deltattabfourthree}{$0.02869^{+0.00075}_{-0.00072}$}
\newcommand{\tautabfourthree}{$0.01220^{+0.00018}_{-0.00013}$}
\newcommand{\tonefourtabfourthree}{$0.08992\pm0.00014$}
\newcommand{\tfwhmtabfourthree}{$0.07770^{+0.00017}_{-0.00018}$}
\newcommand{\ruonetabfourthree}{$0.460\pm0.041$}
\newcommand{\rutwotabfourthree}{$0.151^{+0.075}_{-0.076}$}
\newcommand{\zuonetabfourthree}{$0.313\pm0.025$}
\newcommand{\zutwotabfourthree}{$0.218^{+0.056}_{-0.058}$}
\newcommand{\tuonetabfourthree}{$0.365\pm0.040$}
\newcommand{\tutwotabfourthree}{$0.139^{+0.074}_{-0.075}$}
\newcommand{\rptabfourfour}{$1.339^{+0.023}_{-0.021}$}
\newcommand{\mptabfourfour}{$1.207^{+0.073}_{-0.071}$}
\newcommand{\atabfourfour}{$0.02284^{+0.00040}_{-0.00037}$}
\newcommand{\teqtabfourfour}{$1637^{+20}_{-19}$}
\newcommand{\tcirctabfourfour}{$0.00279\pm0.00018$}
\newcommand{\rhoptabfourfour}{$0.623\pm0.034$}
\newcommand{\loggptabfourfour}{$3.222^{+0.021}_{-0.023}$}
\newcommand{\favetabfourfour}{$1.629^{+0.081}_{-0.075}$}
\newcommand{\msinitabfourfour}{$1.206^{+0.073}_{-0.071}$}
\newcommand{\periodtabfourfour}{$1.338231513\pm0.000000019$}
\newcommand{\tctabfourfour}{$2454697.797524\pm0.000023$}
\newcommand{\tttabfourfour}{$2454697.797524\pm0.000023$}
\newcommand{\tstabfourfour}{$2454698.466640\pm0.000023$}
\newcommand{\tzerotabfourfour}{$2455329.442798\pm0.000022$}
\newcommand{\itabfourfour}{$88.89^{+0.65}_{-0.51}$}
\newcommand{\btabfourfour}{$0.106^{+0.048}_{-0.062}$}
\newcommand{\ktabfourfour}{$240\pm12$}
\newcommand{\ptabfourfour}{$0.15348^{+0.00046}_{-0.00039}$}
\newcommand{\artabfourfour}{$5.482^{+0.019}_{-0.026}$}
\newcommand{\deltatabfourfour}{$0.02355^{+0.00014}_{-0.00012}$}
\newcommand{\deltartabfourfour}{$0.03043^{+0.00086}_{-0.00082}$}
\newcommand{\deltaztabfourfour}{$0.02782^{+0.00049}_{-0.00046}$}
\newcommand{\deltattabfourfour}{$0.02868^{+0.00076}_{-0.00071}$}
\newcommand{\tautabfourfour}{$0.01220^{+0.00017}_{-0.00012}$}
\newcommand{\tonefourtabfourfour}{$0.08992\pm0.00014$}
\newcommand{\tfwhmtabfourfour}{$0.07770^{+0.00017}_{-0.00018}$}
\newcommand{\ruonetabfourfour}{$0.460^{+0.041}_{-0.042}$}
\newcommand{\rutwotabfourfour}{$0.152^{+0.076}_{-0.075}$}
\newcommand{\zuonetabfourfour}{$0.313^{+0.025}_{-0.024}$}
\newcommand{\zutwotabfourfour}{$0.219^{+0.055}_{-0.057}$}
\newcommand{\tuonetabfourfour}{$0.365\pm0.040$}
\newcommand{\tutwotabfourfour}{$0.140^{+0.074}_{-0.076}$}
\begin{turnpage}
  \begin{table*}
     \centering
     \caption{Median values and 68\% confidence interval for the WASP-4 planet fits including the transit}
     \label{tab:wasp4}
     \begin{tabular}{llcccc}
	    \toprule
     \colhead{~~~Parameter} & \colhead{Units} &\colhead{Transit}&\colhead{Transit+SED}&\colhead{MIST+Transit}&\colhead{MIST+Transit+SED}\\
     \toprule
       ~~~~$P$\dotfill&Period (days)\dotfill&\periodtabfourone&\periodtabfourtwo&\periodtabfourthree&\periodtabfourfour\\
       ~~~~$R_P$\dotfill&Radius (\rj)\dotfill&\rptabfourone&\rptabfourtwo&\rptabfourthree&\rptabfourfour\\
       ~~~~$M_P$\dotfill&Mass (\mj)\dotfill&\mptabfourone&\mptabfourtwo&\mptabfourthree&\mptabfourfour\\
       ~~~~$T_C$\dotfill&Time of conjunction$^4$ (\bjdtdb)\dotfill&\tctabfourone&\tctabfourtwo&\tctabfourthree&\tctabfourfour\\
       ~~~~$T_T$\dotfill&Time of min proj sep$^5$ (\bjdtdb)\dotfill&\tttabfourone&\tttabfourtwo&\tttabfourthree&\tttabfourfour\\
       ~~~~$T_0$\dotfill&Optimal conj Time$^6$ (\bjdtdb)\dotfill&\tzerotabfourone&\tzerotabfourtwo&\tzerotabfourthree&\tzerotabfourfour\\
       ~~~~$a$\dotfill&Semi-major axis (AU)\dotfill&\atabfourone&\atabfourtwo&\atabfourthree&\atabfourfour\\
       ~~~~$i$\dotfill&Inclination (Degrees)\dotfill&\itabfourone&\itabfourtwo&\itabfourthree&\itabfourfour\\
       ~~~~$T_{\rm eq}$\dotfill&Equilibrium temperature$^7$ (K)\dotfill&\teqtabfourone&\teqtabfourtwo&\teqtabfourthree&\teqtabfourfour\\
       ~~~~$\tau_{\rm circ}$\dotfill&Tidal circ timescale (Gyr)\dotfill&\tcirctabfourone&\tcirctabfourtwo&\tcirctabfourthree&\tcirctabfourfour\\
       ~~~~$K$\dotfill&RV semi-amplitude (m/s)\dotfill&\ktabfourone&\ktabfourtwo&\ktabfourthree&\ktabfourfour\\
       ~~~~$R_P/R_*$\dotfill&Radius of planet in stellar radii\dotfill&\ptabfourone&\ptabfourtwo&\ptabfourthree&\ptabfourfour\\
       ~~~~$a/R_*$\dotfill&Semi-major axis in stellar radii\dotfill&\artabfourone&\artabfourtwo&\artabfourthree&\artabfourfour\\
       ~~~~$\delta$\dotfill&$(R_P/R_*)^2$\dotfill&\deltatabfourone&\deltatabfourtwo&\deltatabfourthree&\deltatabfourfour\\
       ~~~~$\delta_{\rm R}$\dotfill&Transit depth in R (fraction)\dotfill&\deltartabfourone&\deltartabfourtwo&\deltartabfourthree&\deltartabfourfour\\
       ~~~~$\delta_{\rm z'}$\dotfill&Transit depth in z' (fraction)\dotfill&\deltaztabfourone&\deltaztabfourtwo&\deltaztabfourthree&\deltaztabfourfour\\
       ~~~~$\delta_{\rm TESS}$\dotfill&Transit depth in TESS (fraction)\dotfill&\deltattabfourone&\deltattabfourtwo&\deltattabfourthree&\deltattabfourfour\\
       ~~~~$\tau$\dotfill&Ingress/egress transit duration (days)\dotfill&\tautabfourone&\tautabfourtwo&\tautabfourthree&\tautabfourfour\\
       ~~~~$T_{14}$\dotfill&Total transit duration (days)\dotfill&\tonefourtabfourone&\tonefourtabfourtwo&\tonefourtabfourthree&\tonefourtabfourfour\\
       ~~~~$T_{FWHM}$\dotfill&FWHM transit duration (days)\dotfill&\tfwhmtabfourone&\tfwhmtabfourtwo&\tfwhmtabfourthree&\tfwhmtabfourfour\\
       ~~~~$b$\dotfill&Transit impact parameter\dotfill&\btabfourone&\btabfourtwo&\btabfourthree&\btabfourfour\\
       ~~~~$\rho_P$\dotfill&Density (cgs)\dotfill&\rhoptabfourone&\rhoptabfourtwo&\rhoptabfourthree&\rhoptabfourfour\\
       ~~~~$logg_P$\dotfill&Surface gravity (cgs)\dotfill&\loggptabfourone&\loggptabfourtwo&\loggptabfourthree&\loggptabfourfour\\
       ~~~~$\fave$\dotfill&Incident Flux (\fluxcgs)\dotfill&\favetabfourone&\favetabfourtwo&\favetabfourthree&\favetabfourfour\\
       ~~~~$T_S$\dotfill&Time of eclipse (\bjdtdb)\dotfill&\tstabfourone&\tstabfourtwo&\tstabfourthree&\tstabfourfour\\
       ~~~~$M_P\sin{i}$\dotfill&Minimum mass (\mj)\dotfill&\msinitabfourone&\msinitabfourtwo&\msinitabfourthree&\msinitabfourfour\\
       ~~~~$u_1$\dotfill&R linear limb-darkening coeff\dotfill&\ruonetabfourone&\ruonetabfourtwo&\ruonetabfourthree&\ruonetabfourfour\\
       ~~~~$u_2$\dotfill&R quadratic limb-darkening coeff\dotfill&\rutwotabfourone&\rutwotabfourtwo&\rutwotabfourthree&\rutwotabfourfour\\
       ~~~~$u_1$\dotfill&z' linear limb-darkening coeff\dotfill&\zuonetabfourone&\zuonetabfourtwo&\zuonetabfourthree&\zuonetabfourfour\\
       ~~~~$u_2$\dotfill&z' quadratic limb-darkening coeff\dotfill&\zutwotabfourone&\zutwotabfourtwo&\zutwotabfourthree&\zutwotabfourfour\\
       ~~~~$u_1$\dotfill&TESS linear limb-darkening coeff\dotfill&\tuonetabfourone&\tuonetabfourtwo&\tuonetabfourthree&\tuonetabfourfour\\
       ~~~~$u_2$\dotfill&TESS quadratic limb-darkening coeff\dotfill&\tutwotabfourone&\tutwotabfourtwo&\tutwotabfourthree&\tutwotabfourfour\\
    \hline
    \end{tabular}
    \tablenotetext{}{See Table 3 in \citet{Eastman:2019} for a detailed description of all parameters}
    \tablenotetext{4}{Time of conjunction is commonly reported as the "transit time"}
    \tablenotetext{5}{Time of minimum projected separation is a more correct "transit time"}
    \tablenotetext{6}{Optimal time of conjunction minimizes the covariance between $T_C$ and Period}
    \tablenotetext{7}{Assumes no albedo and perfect redistribution}
  \end{table*}
\end{turnpage}


==> tab5.tex <==
\newcommand{\rptabfiveone}{$1.345^{+0.069}_{-0.070}$}
\newcommand{\mptabfiveone}{$1.19^{+0.14}_{-0.12}$}
\newcommand{\atabfiveone}{$0.0229\pm0.0012$}
\newcommand{\teqtabfiveone}{$1639\pm62$}
\newcommand{\tcirctabfiveone}{$0.00281^{+0.00046}_{-0.00039}$}
\newcommand{\rhoptabfiveone}{$0.609^{+0.12}_{-0.099}$}
\newcommand{\loggptabfiveone}{$3.214^{+0.061}_{-0.062}$}
\newcommand{\favetabfiveone}{$1.64^{+0.26}_{-0.23}$}
\newcommand{\msinitabfiveone}{$1.19^{+0.14}_{-0.12}$}
\newcommand{\rptabfivetwo}{$1.330^{+0.073}_{-0.061}$}
\newcommand{\mptabfivetwo}{$1.199^{+0.078}_{-0.074}$}
\newcommand{\atabfivetwo}{$0.0227^{+0.0012}_{-0.0010}$}
\newcommand{\teqtabfivetwo}{$1643^{+55}_{-57}$}
\newcommand{\tcirctabfivetwo}{$0.00277^{+0.00027}_{-0.00025}$}
\newcommand{\rhoptabfivetwo}{$0.630^{+0.094}_{-0.088}$}
\newcommand{\loggptabfivetwo}{$3.224^{+0.044}_{-0.046}$}
\newcommand{\favetabfivetwo}{$1.66^{+0.23}_{-0.22}$}
\newcommand{\msinitabfivetwo}{$1.198^{+0.078}_{-0.074}$}
\newcommand{\rptabfivethree}{$1.330^{+0.066}_{-0.057}$}
\newcommand{\mptabfivethree}{$1.19^{+0.14}_{-0.12}$}
\newcommand{\atabfivethree}{$0.02268^{+0.0011}_{-0.00097}$}
\newcommand{\teqtabfivethree}{$1642^{+36}_{-38}$}
\newcommand{\tcirctabfivethree}{$0.00278^{+0.00045}_{-0.00039}$}
\newcommand{\rhoptabfivethree}{$0.627^{+0.11}_{-0.097}$}
\newcommand{\loggptabfivethree}{$3.222\pm0.059$}
\newcommand{\favetabfivethree}{$1.65\pm0.15$}
\newcommand{\msinitabfivethree}{$1.19^{+0.14}_{-0.12}$}
\newcommand{\rptabfivefour}{$1.323^{+0.053}_{-0.047}$}
\newcommand{\mptabfivefour}{$1.213^{+0.078}_{-0.074}$}
\newcommand{\atabfivefour}{$0.02257^{+0.00090}_{-0.00081}$}
\newcommand{\teqtabfivefour}{$1646\pm31$}
\newcommand{\tcirctabfivefour}{$0.00271^{+0.00027}_{-0.00025}$}
\newcommand{\rhoptabfivefour}{$0.648^{+0.087}_{-0.082}$}
\newcommand{\loggptabfivefour}{$3.234^{+0.042}_{-0.044}$}
\newcommand{\favetabfivefour}{$1.67^{+0.13}_{-0.12}$}
\newcommand{\msinitabfivefour}{$1.213^{+0.078}_{-0.074}$}
\newcommand{\periodref}{$1.338231512\pm0.000000019$}
\newcommand{\tcref}{$2454697.797524\pm0.000024$}
\newcommand{\ttref}{$2454697.797524\pm0.000024$}
\newcommand{\tsref}{$2454698.466639\pm0.000024$}
\newcommand{\tzeroref}{$2455337.472187\pm0.000022$}
\newcommand{\iref}{$88.87^{+0.67}_{-0.51}$}
\newcommand{\bref}{$0.108^{+0.048}_{-0.064}$}
\newcommand{\kref}{$240\pm12$}
\newcommand{\pref}{$0.15348^{+0.00047}_{-0.00039}$}
\newcommand{\arref}{$5.481^{+0.020}_{-0.026}$}
\newcommand{\deltaref}{$0.02356^{+0.00014}_{-0.00012}$}
\newcommand{\deltarref}{$0.03042^{+0.00086}_{-0.00081}$}
\newcommand{\deltazref}{$0.02781^{+0.00049}_{-0.00046}$}
\newcommand{\deltatref}{$0.02867^{+0.00076}_{-0.00072}$}
\newcommand{\tauref}{$0.01220^{+0.00017}_{-0.00013}$}
\newcommand{\tonefourref}{$0.08992\pm0.00014$}
\newcommand{\tfwhmref}{$0.07770^{+0.00017}_{-0.00018}$}
\newcommand{\ruoneref}{$0.460\pm0.041$}
\newcommand{\rutworef}{$0.152^{+0.075}_{-0.076}$}
\newcommand{\zuoneref}{$0.312^{+0.025}_{-0.024}$}
\newcommand{\zutworef}{$0.219^{+0.055}_{-0.057}$}
\newcommand{\tuoneref}{$0.364^{+0.041}_{-0.040}$}
\newcommand{\tutworef}{$0.141^{+0.075}_{-0.076}$}
\begin{turnpage}
  \begin{table*}
     \centering
     \caption{Median values and 68\% confidence interval for WASP-4b planet fits, propagating the transit observables with the star only fits}
     \label{tab:wasp4}
     \begin{tabular}{llcccc}
	    \toprule
     \colhead{~~~Parameter} & \colhead{Units} &\colhead{None}&\colhead{MIST}&\colhead{SED}&\colhead{MIST+SED}\\
     \toprule
       ~~~~$P$\dotfill&Period (days)\dotfill&\multicolumn{4}{c}{\periodref}\\
       ~~~~$R_P$\dotfill&Radius (\rj)\dotfill&\rptabfiveone&\rptabfivetwo&\rptabfivethree&\rptabfivefour\\
       ~~~~$M_P$\dotfill&Mass (\mj)\dotfill&\mptabfiveone&\mptabfivetwo&\mptabfivethree&\mptabfivefour\\
       ~~~~$T_C$\dotfill&Time of conjunction$^4$ (\bjdtdb)\dotfill&\multicolumn{4}{c}{\tcref}\\
       ~~~~$T_T$\dotfill&Time of min proj sep$^5$ (\bjdtdb)\dotfill&\multicolumn{4}{c}{\ttref}\\
       ~~~~$T_0$\dotfill&Optimal conj Time$^6$ (\bjdtdb)\dotfill&\multicolumn{4}{c}{\tzeroref}\\
       ~~~~$a$\dotfill&Semi-major axis (AU)\dotfill&\atabfiveone&\atabfivetwo&\atabfivethree&\atabfivefour\\
       ~~~~$i$\dotfill&Inclination (Degrees)\dotfill&\multicolumn{4}{c}{\iref}\\
       ~~~~$T_{\rm eq}$\dotfill&Equilibrium temperature$^7$ (K)\dotfill&\teqtabfiveone&\teqtabfivetwo&\teqtabfivethree&\teqtabfivefour\\
       ~~~~$\tau_{\rm circ}$\dotfill&Tidal circ timescale (Gyr)\dotfill&\tcirctabfiveone&\tcirctabfivetwo&\tcirctabfivethree&\tcirctabfivefour\\
       ~~~~$K$\dotfill&RV semi-amplitude (m/s)\dotfill&\multicolumn{4}{c}{\kref}\\
       ~~~~$R_P/R_*$\dotfill&Radius of planet in stellar radii\dotfill&\multicolumn{4}{c}{\pref}\\
       ~~~~$a/R_*$\dotfill&Semi-major axis in stellar radii\dotfill&\multicolumn{4}{c}{\arref}\\
       ~~~~$\delta$\dotfill&$(R_P/R_*)^2$\dotfill&\multicolumn{4}{c}{\deltaref}\\
       ~~~~$\delta_{\rm R}$\dotfill&Transit depth in R (fraction)\dotfill&\multicolumn{4}{c}{\deltarref}\\
       ~~~~$\delta_{\rm z'}$\dotfill&Transit depth in z' (fraction)\dotfill&\multicolumn{4}{c}{\deltazref}\\
       ~~~~$\delta_{\rm TESS}$\dotfill&Transit depth in TESS (fraction)\dotfill&\multicolumn{4}{c}{\deltatref}\\
       ~~~~$\tau$\dotfill&Ingress/egress transit duration (days)\dotfill&\multicolumn{4}{c}{\tauref}\\
       ~~~~$T_{14}$\dotfill&Total transit duration (days)\dotfill&\multicolumn{4}{c}{\tonefourref}\\
       ~~~~$T_{FWHM}$\dotfill&FWHM transit duration (days)\dotfill&\multicolumn{4}{c}{\tfwhmref}\\
       ~~~~$b$\dotfill&Transit impact parameter\dotfill&\multicolumn{4}{c}{\bref}\\
       ~~~~$\rho_P$\dotfill&Density (cgs)\dotfill&\rhoptabfiveone&\rhoptabfivetwo&\rhoptabfivethree&\rhoptabfivefour\\
       ~~~~$logg_P$\dotfill&Surface gravity (cgs)\dotfill&\loggptabfiveone&\loggptabfivetwo&\loggptabfivethree&\loggptabfivefour\\
       ~~~~$\fave$\dotfill&Incident Flux (\fluxcgs)\dotfill&\favetabfiveone&\favetabfivetwo&\favetabfivethree&\favetabfivefour\\
       ~~~~$T_S$\dotfill&Time of eclipse (\bjdtdb)\dotfill&\multicolumn{4}{c}{\tsref}\\
       ~~~~$M_P\sin{i}$\dotfill&Minimum mass (\mj)\dotfill&\msinitabfiveone&\msinitabfivetwo&\msinitabfivethree&\msinitabfivefour\\
       ~~~~$u_1$\dotfill&R linear limb-darkening coeff\dotfill&\multicolumn{4}{c}{\ruoneref}\\
       ~~~~$u_2$\dotfill&R quadratic limb-darkening coeff\dotfill&\multicolumn{4}{c}{\rutworef}\\
       ~~~~$u_1$\dotfill&z' linear limb-darkening coeff\dotfill&\multicolumn{4}{c}{\zuoneref}\\
       ~~~~$u_2$\dotfill&z' quadratic limb-darkening coeff\dotfill&\multicolumn{4}{c}{\zutworef}\\
       ~~~~$u_1$\dotfill&TESS linear limb-darkening coeff\dotfill&\multicolumn{4}{c}{\tuoneref}\\
       ~~~~$u_2$\dotfill&TESS quadratic limb-darkening coeff\dotfill&\multicolumn{4}{c}{\tutworef}\\
    \hline
    \end{tabular}
    \tablenotetext{}{See Table 3 in \citet{Eastman:2019} for a detailed description of all parameters}
    \tablenotetext{4}{Time of conjunction is commonly reported as the "transit time"}
    \tablenotetext{5}{Time of minimum projected separation is a more correct "transit time"}
    \tablenotetext{6}{Optimal time of conjunction minimizes the covariance between $T_C$ and Period}
    \tablenotetext{7}{Assumes no albedo and perfect redistribution}
  \end{table*}
\end{turnpage}


==> wasp4.all.tex <==
%\begin{landscape}
%\startlongtable
%\begin{deluxetable*}{llcccccccc}
%\tablecaption{Median values and 68\% confidence interval for WASP-4b.\label{tab:wasp4}}
%\tablehead{\colhead{~~~Parameter} & \colhead{Units} & \colhead{None} & \colhead{SED} & \colhead{MIST} & \colhead{MIST+SED} & \colhead{Transit} & \colhead{Transit+SED} & \colhead{MIST+Transit} & \colhead{MIST+Transit+SED}}
%\startdata


\begin{turnpage}

\begin{table*}
	\centering
	\caption{Median values and 68\% confidence interval for the WASP-4 host star}
	\label{tab:wasp4}
	\begin{tabular}{llcccccccc}
	\toprule	\colhead{~~~Parameter} & \colhead{Units} & \colhead{None} & \colhead{SED} & \colhead{MIST} & \colhead{MIST+SED} & \colhead{Transit} & \colhead{Transit+SED} & \colhead{MIST+Transit} & \colhead{MIST+Transit+SED} \\
	\toprule

%smallskip\\\multicolumn{2}{l}{Stellar Parameters:}&\smallskip\\
~~~~$M_*$\dotfill&Mass (\msun)\dotfill &$0.88^{+0.15}_{-0.12}$&$0.87^{+0.15}_{-0.13}$&$0.880^{+0.054}_{-0.048}$&$0.895^{+0.048}_{-0.044}$&$0.91\pm0.14$&$0.87^{+0.12}_{-0.10}$&$0.890^{+0.068}_{-0.056}$&$0.885^{+0.044}_{-0.039}$\\
~~~~$R_*$\dotfill&Radius (\rsun)\dotfill &$0.899^{+0.047}_{-0.046}$&$0.889^{+0.041}_{-0.037}$&$0.888^{+0.048}_{-0.040}$&$0.885^{+0.033}_{-0.029}$&$0.903^{+0.043}_{-0.048}$&$0.890^{+0.040}_{-0.036}$&$0.898^{+0.023}_{-0.020}$&$0.896^{+0.015}_{-0.013}$\\
~~~~$L_*$\dotfill&Luminosity (\lsun)\dotfill &$0.629^{+0.12}_{-0.100}$&$0.625^{+0.030}_{-0.026}$&$0.63^{+0.12}_{-0.11}$&$0.623^{+0.028}_{-0.026}$&$0.632^{+0.12}_{-0.098}$&$0.624^{+0.026}_{-0.025}$&$0.65\pm0.11$&$0.625^{+0.026}_{-0.024}$\\
~~~~$\rho_*$\dotfill&Density (cgs)\dotfill &$1.70^{+0.38}_{-0.31}$&$1.75^{+0.37}_{-0.31}$&$1.78^{+0.22}_{-0.24}$&$1.83\pm0.22$&$1.737^{+0.019}_{-0.024}$&$1.738^{+0.019}_{-0.024}$&$1.739^{+0.019}_{-0.024}$&$1.739^{+0.018}_{-0.024}$\\
~~~~$\log{g}$\dotfill&Surface gravity (cgs)\dotfill &$4.472^{+0.074}_{-0.073}$&$4.480^{+0.075}_{-0.073}$&$4.487^{+0.036}_{-0.043}$&$4.496^{+0.037}_{-0.041}$&$4.484^{+0.020}_{-0.024}$&$4.478^{+0.019}_{-0.018}$&$4.4816^{+0.011}_{-0.0099}$&$4.4808^{+0.0078}_{-0.0076}$\\
~~~~$T_{\rm eff}$\dotfill&Effective Temp (K)\dotfill &$5420\pm210$&$5450^{+110}_{-120}$&$5440\pm180$&$5450^{+90}_{-93}$&$5420\pm210$&$5440\pm110$&$5470^{+170}_{-200}$&$5421^{+61}_{-59}$\\
~~~~$[{\rm Fe/H}]$\dotfill&Metallicity (dex)\dotfill &$-0.029^{+0.089}_{-0.092}$&$0.013^{+0.087}_{-0.083}$&$-0.024^{+0.089}_{-0.088}$&$0.015^{+0.081}_{-0.079}$&$-0.030\pm0.090$&$0.013^{+0.084}_{-0.079}$&$-0.020^{+0.089}_{-0.088}$&$0.014^{+0.081}_{-0.077}$\\
~~~~$R_{*,SED}$\dotfill&Radius$^{1}$ (\rsun)\dotfill &--&$0.883\pm0.017$&--&$0.881^{+0.017}_{-0.016}$&--&$0.883\pm0.016$&--&$0.883^{+0.016}_{-0.015}$\\
~~~~$F_{Bol}$\dotfill&Bol Flux $\times 10^{10}$ (cgs)\dotfill &--&$2.866^{+0.091}_{-0.078}$&--&$2.864^{+0.091}_{-0.077}$&--&$2.865^{+0.080}_{-0.073}$&--&$2.865^{+0.081}_{-0.073}$\\
~~~~$T_{\rm eff,SED}$\dotfill&Effective Temp$^{1}$ (K)\dotfill &--&$5462^{+34}_{-31}$&--&$5463^{+32}_{-31}$&--&$5460^{+30}_{-29}$&--&$5460^{+30}_{-29}$\\
~~~~$[{\rm Fe/H}]_{SED}$\dotfill&Metallicity (dex)\dotfill &--&$0.043^{+0.11}_{-0.097}$&--&$0.044^{+0.11}_{-0.095}$&--&$0.044^{+0.11}_{-0.090}$&--&$0.042^{+0.10}_{-0.088}$\\
~~~~$A_V$\dotfill&V-band ext (mag)\dotfill &--&$0.023^{+0.014}_{-0.016}$&--&$0.023^{+0.014}_{-0.016}$&--&$0.023^{+0.014}_{-0.015}$&--&$0.023^{+0.014}_{-0.015}$\\
~~~~$\sigma_{SED}$\dotfill&SED phot err scale \dotfill &--&$1.02^{+0.43}_{-0.24}$&--&$1.00^{+0.39}_{-0.23}$&--&$0.97^{+0.33}_{-0.21}$&--&$0.97^{+0.33}_{-0.21}$\\
~~~~$\varpi$\dotfill&Parallax (mas)\dotfill &--&$3.788^{+0.064}_{-0.061}$&--&$3.793^{+0.061}_{-0.060}$&--&$3.788\pm0.060$&--&$3.788\pm0.059$\\
~~~~$d$\dotfill&Distance (pc)\dotfill &--&$264.0^{+4.3}_{-4.4}$&--&$263.6^{+4.2}_{-4.1}$&--&$264.0^{+4.2}_{-4.1}$&--&$264.0^{+4.2}_{-4.0}$\\
~~~~$[{\rm Fe/H}]_{0}$\dotfill&Initial Metallicity$^{2}$ \dotfill &--&--&$0.00\pm0.10$&$0.031^{+0.098}_{-0.100}$&--&--&$0.01\pm0.10$&$0.036^{+0.096}_{-0.095}$\\
~~~~$Age$\dotfill&Age (Gyr)\dotfill &--&--&$7.2^{+4.3}_{-3.7}$&$6.3^{+4.6}_{-3.8}$&--&--&$6.9^{+4.3}_{-4.0}$&$7.6^{+3.3}_{-3.4}$\\
~~~~$EEP$\dotfill&Equal Evol Phase$^{3}$ \dotfill &--&--&$352^{+35}_{-18}$&$350^{+36}_{-25}$&--&--&$354^{+30}_{-21}$&$359^{+26}_{-20}$\\
	\hline
	\end{tabular}
\tablenotetext{}{See Table 3 in \citet{Eastman:2019} for a detailed description of all parameters\hfill\hfill}
\tablenotetext{1}{This value ignores the systematic error and is for reference only}
\tablenotetext{2}{The metallicity of the star at birth}
\tablenotetext{3}{Corresponds to static points in a star's evolutionary history. See \S2 in \citet{Dotter:2016}.}

\end{table*}
	
\end{turnpage}


\bigskip
\clearpage

\begin{turnpage}
\begin{table*}
	\centering
	\caption{Median values and 68\% confidence interval for the WASP-4b planet}
	\label{tab:wasp4b}
	\begin{tabular}{llcccc}
	\toprule	\colhead{~~~Parameter} & \colhead{Units} &  \colhead{Transit} & \colhead{Transit+SED} & \colhead{MIST+Transit} & \colhead{MIST+Transit+SED} \\
	\toprule
%smallskip\\\multicolumn{2}{l}{Planetary Parameters:}\smallskip\\
~~~~$P$\dotfill&Period (days)\dotfill &$1.338231512\pm0.000000019$&$1.338231512\pm0.000000019$&$1.338231513\pm0.000000019$&$1.338231512\pm0.000000019$\\
~~~~$R_P$\dotfill&Radius (\rj)\dotfill &$1.348^{+0.064}_{-0.071}$&$1.330^{+0.059}_{-0.054}$&$1.341^{+0.034}_{-0.030}$&$1.338^{+0.022}_{-0.021}$\\
~~~~$M_P$\dotfill&Mass (\mj)\dotfill &$1.22\pm0.13$&$1.19^{+0.12}_{-0.11}$&$1.211^{+0.085}_{-0.080}$&$1.205^{+0.071}_{-0.069}$\\
~~~~$T_C$\dotfill&Time of conjunction$^{4}$ (\bjdtdb)\dotfill &$2454697.797524\pm0.000024$&$2454697.797525\pm0.000024$&$2454697.797524^{+0.000024}_{-0.000023}$&$2454697.797525^{+0.000023}_{-0.000024}$\\
~~~~$T_T$\dotfill&Time of min proj sep$^{5}$ (\bjdtdb)\dotfill &$2454697.797524\pm0.000024$&$2454697.797525\pm0.000024$&$2454697.797524^{+0.000024}_{-0.000023}$&$2454697.797525^{+0.000023}_{-0.000024}$\\
~~~~$T_0$\dotfill&Optimal conj Time$^{6}$ (\bjdtdb)\dotfill &$2455334.795723\pm0.000022$&$2455349.516272\pm0.000022$&$2455326.766335\pm0.000022$&$2455345.501576\pm0.000022$\\
~~~~$a$\dotfill&Semi-major axis (AU)\dotfill &$0.0230^{+0.0011}_{-0.0012}$&$0.02269^{+0.0010}_{-0.00091}$&$0.02287^{+0.00057}_{-0.00049}$&$0.02282^{+0.00037}_{-0.00034}$\\
~~~~$i$\dotfill&Inclination (Degrees)\dotfill &$88.86^{+0.65}_{-0.51}$&$88.88^{+0.66}_{-0.50}$&$88.90^{+0.65}_{-0.51}$&$88.91^{+0.66}_{-0.52}$\\
~~~~$T_{eq}$\dotfill&Equilibrium temperature$^{7}$ (K)\dotfill &$1638^{+64}_{-62}$&$1642^{+33}_{-34}$&$1652^{+53}_{-60}$&$1637\pm18$\\
~~~~$\tau_{\rm circ}$\dotfill&Tidal circ timescale (Gyr)\dotfill &$0.00277^{+0.00021}_{-0.00020}$&$0.00280^{+0.00020}_{-0.00019}$&$0.00278^{+0.00017}_{-0.00018}$&$0.00279^{+0.00016}_{-0.00017}$\\
~~~~$K$\dotfill&RV semi-amplitude (m/s)\dotfill &$240\pm12$&$240\pm12$&$240\pm12$&$240^{+11}_{-12}$\\
~~~~$R_P/R_*$\dotfill&Radius of planet in stellar radii \dotfill &$0.15349^{+0.00047}_{-0.00040}$&$0.15348^{+0.00046}_{-0.00039}$&$0.15347^{+0.00046}_{-0.00039}$&$0.15346^{+0.00047}_{-0.00039}$\\
~~~~$a/R_*$\dotfill&Semi-major axis in stellar radii \dotfill &$5.481^{+0.020}_{-0.026}$&$5.482^{+0.020}_{-0.026}$&$5.483^{+0.019}_{-0.026}$&$5.483^{+0.019}_{-0.026}$\\
~~~~$\delta$\dotfill&$\left(R_P/R_*\right)^2$ \dotfill &$0.02356^{+0.00014}_{-0.00012}$&$0.02355^{+0.00014}_{-0.00012}$&$0.02355^{+0.00014}_{-0.00012}$&$0.02355^{+0.00014}_{-0.00012}$\\
~~~~$\delta_{\rm R}$\dotfill&Transit depth in R (fraction)\dotfill &$0.03043^{+0.00087}_{-0.00082}$&$0.03042^{+0.00086}_{-0.00080}$&$0.03043^{+0.00085}_{-0.00081}$&$0.03042^{+0.00085}_{-0.00081}$\\
~~~~$\delta_{\rm z'}$\dotfill&Transit depth in z' (fraction)\dotfill &$0.02782^{+0.00049}_{-0.00047}$&$0.02781^{+0.00049}_{-0.00046}$&$0.02782^{+0.00049}_{-0.00046}$&$0.02781^{+0.00049}_{-0.00046}$\\
~~~~$\delta_{\rm TESS}$\dotfill&Transit depth in TESS (fraction)\dotfill &$0.02869^{+0.00076}_{-0.00072}$&$0.02867^{+0.00076}_{-0.00070}$&$0.02868^{+0.00075}_{-0.00071}$&$0.02866^{+0.00076}_{-0.00071}$\\
~~~~$\tau$\dotfill&Ingress/egress transit duration (days)\dotfill &$0.01221^{+0.00017}_{-0.00013}$&$0.01220^{+0.00017}_{-0.00013}$&$0.01220^{+0.00017}_{-0.00012}$&$0.01219^{+0.00017}_{-0.00012}$\\
~~~~$T_{14}$\dotfill&Total transit duration (days)\dotfill &$0.08992\pm0.00014$&$0.08992\pm0.00014$&$0.08992\pm0.00014$&$0.08992\pm0.00014$\\
~~~~$T_{FWHM}$\dotfill&FWHM transit duration (days)\dotfill &$0.07770^{+0.00017}_{-0.00018}$&$0.07770^{+0.00017}_{-0.00018}$&$0.07770^{+0.00017}_{-0.00018}$&$0.07771^{+0.00017}_{-0.00018}$\\
~~~~$b$\dotfill&Transit Impact parameter \dotfill &$0.109^{+0.048}_{-0.062}$&$0.107^{+0.048}_{-0.063}$&$0.105^{+0.048}_{-0.062}$&$0.104^{+0.049}_{-0.063}$\\
%~~~~$\delta_{S,2.5\mu m}$\dotfill&Blackbody eclipse depth at 2.5$\mu$m (ppm)\dotfill &$1370^{+110}_{-100}$&$1373^{+56}_{-58}$&$1390^{+88}_{-100}$&$1364^{+33}_{-32}$\\
%~~~~$\delta_{S,5.0\mu m}$\dotfill&Blackbody eclipse depth at 5.0$\mu$m (ppm)\dotfill &$3430\pm110$&$3436^{+63}_{-64}$&$3454^{+90}_{-110}$&$3426^{+43}_{-39}$\\
%~~~~$\delta_{S,7.5\mu m}$\dotfill&Blackbody eclipse depth at 7.5$\mu$m (ppm)\dotfill &$4475^{+88}_{-92}$&$4477^{+57}_{-55}$&$4491^{+75}_{-89}$&$4469^{+45}_{-38}$\\
~~~~$\rho_P$\dotfill&Density (cgs)\dotfill &$0.619^{+0.045}_{-0.042}$&$0.626^{+0.042}_{-0.041}$&$0.622\pm0.036$&$0.624^{+0.033}_{-0.034}$\\
~~~~$logg_P$\dotfill&Surface gravity \dotfill &$3.222^{+0.021}_{-0.023}$&$3.222^{+0.021}_{-0.023}$&$3.222^{+0.021}_{-0.023}$&$3.222^{+0.021}_{-0.023}$\\
%~~~~$\Theta$\dotfill&Safronov Number \dotfill &$0.0461^{+0.0033}_{-0.0030}$&$0.0466^{+0.0030}_{-0.0029}$&$0.0462^{+0.0025}_{-0.0026}$&$0.0464\pm0.0024$\\
~~~~$\fave$\dotfill&Incident Flux (\fluxcgs)\dotfill &$1.64^{+0.27}_{-0.24}$&$1.65^{+0.14}_{-0.13}$&$1.69\pm0.23$&$1.631^{+0.074}_{-0.069}$\\
%~~~~$T_P$\dotfill&Time of Periastron (\bjdtdb)\dotfill &$2454697.797524\pm0.000024$&$2454697.797525\pm0.000024$&$2454697.797524^{+0.000024}_{-0.000023}$&$2454697.797525^{+0.000023}_{-0.000024}$\\
~~~~$T_S$\dotfill&Time of eclipse (\bjdtdb)\dotfill &$2454698.466639\pm0.000024$&$2454698.466641\pm0.000024$&$2454698.466640^{+0.000024}_{-0.000023}$&$2454698.466640^{+0.000023}_{-0.000024}$\\
%~~~~$T_A$\dotfill&Time of Ascending Node (\bjdtdb)\dotfill &$2454698.801197\pm0.000024$&$2454698.801199\pm0.000024$&$2454698.801198^{+0.000024}_{-0.000023}$&$2454698.801198^{+0.000023}_{-0.000024}$\\
%~~~~$T_D$\dotfill&Time of Descending Node (\bjdtdb)\dotfill &$2454698.132082\pm0.000024$&$2454698.132083\pm0.000024$&$2454698.132082^{+0.000024}_{-0.000023}$&$2454698.132082^{+0.000023}_{-0.000024}$\\
%~~~~$V_c/V_e$\dotfill& \dotfill &$1.00$&$1.00$&$1.00$&$1.00$\\
~~~~$M_P\sin i$\dotfill&Minimum mass (\mj)\dotfill &$1.22\pm0.13$&$1.19^{+0.12}_{-0.11}$&$1.211^{+0.085}_{-0.080}$&$1.204^{+0.071}_{-0.069}$\\
%~~~~$M_P/M_*$\dotfill&Mass ratio \dotfill &$0.001291^{+0.000092}_{-0.000085}$&$0.001306^{+0.000085}_{-0.000082}$&$0.001295^{+0.000070}_{-0.000071}$&$0.001299^{+0.000066}_{-0.000068}$\\
~~~~$u_{1}$\dotfill&R linear limb-darkening coeff \dotfill &$0.460\pm0.042$&$0.460\pm0.041$&$0.460\pm0.041$&$0.460\pm0.041$\\
~~~~$u_{2}$\dotfill&R quadratic limb-darkening coeff \dotfill &$0.151^{+0.075}_{-0.076}$&$0.152^{+0.074}_{-0.075}$&$0.152^{+0.074}_{-0.075}$&$0.152\pm0.075$\\
~~~~$u_{1}$\dotfill&z' linear limb-darkening coeff \dotfill &$0.313\pm0.025$&$0.312^{+0.025}_{-0.024}$&$0.313^{+0.025}_{-0.024}$&$0.312^{+0.025}_{-0.024}$\\
~~~~$u_{2}$\dotfill&z' quadratic limb-darkening coeff \dotfill &$0.218^{+0.056}_{-0.058}$&$0.220^{+0.055}_{-0.057}$&$0.219^{+0.055}_{-0.057}$&$0.220^{+0.055}_{-0.057}$\\
~~~~$u_{1}$\dotfill&TESS linear limb-darkening coeff \dotfill &$0.365\pm0.041$&$0.364^{+0.041}_{-0.040}$&$0.364\pm0.040$&$0.364\pm0.040$\\
~~~~$u_{2}$\dotfill&TESS quadratic limb-darkening coeff \dotfill &$0.139^{+0.075}_{-0.076}$&$0.141^{+0.073}_{-0.075}$&$0.140\pm0.074$&$0.142^{+0.073}_{-0.076}$\\
%~~~~$d/R_*$\dotfill&Separation at mid transit \dotfill &$5.481^{+0.020}_{-0.026}$&$5.482^{+0.020}_{-0.026}$&$5.483^{+0.019}_{-0.026}$&$5.483^{+0.019}_{-0.026}$\\
%~~~~$P_T$\dotfill&A priori non-grazing transit prob \dotfill &$0.15445^{+0.00066}_{-0.00054}$&$0.15444^{+0.00067}_{-0.00053}$&$0.15441^{+0.00066}_{-0.00052}$&$0.15440^{+0.00065}_{-0.00051}$\\
%~~~~$P_{T,G}$\dotfill&A priori transit prob \dotfill &$0.21043^{+0.0011}_{-0.00080}$&$0.21041^{+0.0011}_{-0.00079}$&$0.21037^{+0.0011}_{-0.00077}$&$0.21035^{+0.0011}_{-0.00075}$\\
%~~~~$\gamma_{\rm rel}$\dotfill&Relative RV Offset (m/s)\dotfill &$57732.6^{+7.2}_{-7.5}$&$57732.7^{+7.1}_{-7.4}$&$57732.7^{+7.3}_{-7.4}$&$57732.6^{+7.1}_{-7.4}$\\
%~~~~$\sigma_J$\dotfill&RV Jitter (m/s)\dotfill &$19.9^{+9.4}_{-7.4}$&$19.8^{+9.3}_{-7.4}$&$19.9^{+9.3}_{-7.4}$&$19.7^{+9.1}_{-7.3}$\\
%~~~~$\sigma_J^2$\dotfill&RV Jitter Variance \dotfill &$400^{+460}_{-240}$&$390^{+460}_{-240}$&$400^{+460}_{-240}$&$390^{+440}_{-230}$\\
%~~~~$\sigma^{2}$\dotfill&Added Variance \dotfill &$0.00000234^{+0.00000035}_{-0.00000031}$&$0.00000235^{+0.00000035}_{-0.00000031}$&$0.00000234^{+0.00000035}_{-0.00000031}$&$0.00000234^{+0.00000035}_{-0.00000031}$\\
%~~~~$F_0$\dotfill&Baseline flux \dotfill &$0.99974\pm0.00013$&$0.99974\pm0.00013$&$0.99974^{+0.00012}_{-0.00013}$&$0.99974\pm0.00013$\\

	\hline
	\end{tabular}

\tablenotetext{}{See Table 3 in \citet{Eastman:2019} for a detailed description of all parameters}
\tablenotetext{4}{Time of conjunction is commonly reported as the "transit time"}
\tablenotetext{5}{Time of minimum projected separation is a more correct "transit time"}
\tablenotetext{6}{Optimal time of conjunction minimizes the covariance between $T_C$ and Period}
\tablenotetext{7}{Assumes no albedo and perfect redistribution}

\end{table*}


\end{turnpage}


%\enddata

%\tablenotetext{1}{This value ignores the systematic error and is for reference only}
%\tablenotetext{2}{The metallicity of the star at birth}
%\tablenotetext{3}{Corresponds to static points in a star's evolutionary history. See \S2 in \citet{Dotter:2016}.}
%\tablenotetext{4}{Time of conjunction is commonly reported as the "transit time"}
%\tablenotetext{5}{Time of minimum projected separation is a more correct "transit time"}
%\tablenotetext{6}{Optimal time of conjunction minimizes the covariance between $T_C$ and Period}
%\tablenotetext{7}{Assumes no albedo and perfect redistribution}
%\end{deluxetable*}
%\end{landscape}

==> wasp4b.tex <==
\startlongtable
\begin{deluxetable*}{lcccccccccccc}
\tablecaption{Median values and 68\% confidence interval for WASP-4b.circ3.\label{tab:wasp4}}
\tablehead{\colhead{~~~Parameter} & \colhead{Units} & \multicolumn{11}{c}{Values}}
\startdata
\smallskip\\\multicolumn{2}{l}{Stellar Parameters:}&\smallskip\\
~~~~$M_*$\dotfill &Mass (\msun)\dotfill &$0.875^{+0.040}_{-0.034}$\\
~~~~$R_*$\dotfill &Radius (\rsun)\dotfill &$0.891^{+0.013}_{-0.012}$\\
~~~~$R_{*,SED}$\dotfill &Radius$^{1}$ (\rsun)\dotfill &$0.890^{+0.014}_{-0.012}$\\
~~~~$L_*$\dotfill &Luminosity (\lsun)\dotfill &$0.634^{+0.023}_{-0.021}$\\
~~~~$F_{Bol}$\dotfill &Bolometric Flux (cgs)\dotfill &$2.893^{+0.076}_{-0.072} \times 10^{-10}$ \\%$0.0000000002893^{+0.0000000000076}_{-0.0000000000072}$\\
~~~~$\rho_*$\dotfill &Density (cgs)\dotfill &$1.745^{+0.010}_{-0.018}$\\
~~~~$\log{g}$\dotfill &Surface gravity (cgs)\dotfill &$4.4800^{+0.0069}_{-0.0064}$\\
~~~~$T_{\rm eff}$\dotfill &Effective Temperature (K)\dotfill &$5452^{+45}_{-43}$\\
~~~~$T_{\rm eff,SED}$\dotfill &Effective Temperature$^{1}$ (K)\dotfill &$5465^{+31}_{-29}$\\
~~~~$[{\rm Fe/H}]$\dotfill &Metallicity (dex)\dotfill &$-0.007^{+0.076}_{-0.058}$\\
~~~~$[{\rm Fe/H}]_{0}$\dotfill &Initial Metallicity$^{2}$ \dotfill &$0.021^{+0.071}_{-0.063}$\\
~~~~$Age$\dotfill &Age (Gyr)\dotfill &$8.3^{+3.0}_{-3.1}$\\
~~~~$EEP$\dotfill &Equal Evolutionary Phase$^{3}$ \dotfill &$365^{+20}_{-19}$\\
~~~~$A_V$\dotfill &V-band extinction (mag)\dotfill &$0.024^{+0.013}_{-0.015}$\\
~~~~$\sigma_{SED}$\dotfill &SED photometry error scaling \dotfill &$1.00^{+0.34}_{-0.22}$\\
~~~~$\varpi$\dotfill &Parallax (mas)\dotfill &$3.777\pm0.055$\\
~~~~$d$\dotfill &Distance (pc)\dotfill &$264.8^{+3.9}_{-3.8}$\\
\smallskip\\\multicolumn{2}{l}{Planetary Parameters:}&b\smallskip\\
~~~~$P$\dotfill &Period (days)\dotfill &$1.338231511^{+0.000000019}_{-0.000000018}$\\
~~~~$R_P$\dotfill &Radius (\rj)\dotfill &$1.328^{+0.020}_{-0.018}$\\
~~~~$M_P$\dotfill &Mass (\mj)\dotfill &$1.197^{+0.071}_{-0.066}$\\
~~~~$T_C$\dotfill &Time of conjunction$^{4}$ (\bjdtdb)\dotfill &$2454697.797525\pm0.000024$\\
~~~~$T_T$\dotfill &Time of minimum projected separation$^{5}$ (\bjdtdb)\dotfill &$2454697.797525\pm0.000024$\\
~~~~$T_0$\dotfill &Optimal conjunction Time$^{6}$ (\bjdtdb)\dotfill &$2458258.831576^{+0.000047}_{-0.000045}$\\
~~~~$a$\dotfill &Semi-major axis (AU)\dotfill &$0.02274^{+0.00034}_{-0.00030}$\\
~~~~$i$\dotfill &Inclination (Degrees)\dotfill &$89.31^{+0.46}_{-0.48}$\\
~~~~$T_{eq}$\dotfill &Equilibrium temperature$^{7}$ (K)\dotfill &$1646^{+14}_{-13}$\\
~~~~$\tau_{\rm circ}$\dotfill &Tidal circularization timescale (Gyr)\dotfill &$0.00285\pm0.00016$\\
~~~~$K$\dotfill &RV semi-amplitude (m/s)\dotfill &$240\pm12$\\
~~~~$R_P/R_*$\dotfill &Radius of planet in stellar radii \dotfill &$0.15309^{+0.00025}_{-0.00021}$\\
~~~~$a/R_*$\dotfill &Semi-major axis in stellar radii \dotfill &$5.489^{+0.011}_{-0.019}$\\
~~~~$\delta$\dotfill &$\left(R_P/R_*\right)^2$ \dotfill &$0.023436^{+0.000076}_{-0.000064}$\\
~~~~$\delta_{\rm R}$\dotfill &Transit depth in R (fraction)\dotfill &$0.02958^{+0.00027}_{-0.00026}$\\
~~~~$\delta_{\rm z'}$\dotfill &Transit depth in z' (fraction)\dotfill &$0.02750\pm0.00021$\\
~~~~$\delta_{\rm TESS}$\dotfill &Transit depth in TESS (fraction)\dotfill &$0.02795^{+0.00026}_{-0.00025}$\\
~~~~$\tau$\dotfill &Ingress/egress transit duration (days)\dotfill &$0.012107^{+0.00011}_{-0.000051}$\\
~~~~$T_{14}$\dotfill &Total transit duration (days)\dotfill &$0.090005^{+0.00010}_{-0.000100}$\\
~~~~$T_{FWHM}$\dotfill &FWHM transit duration (days)\dotfill &$0.077877^{+0.000094}_{-0.000097}$\\
~~~~$b$\dotfill &Transit Impact parameter \dotfill &$0.066^{+0.046}_{-0.044}$\\
~~~~$\delta_{S,2.5\mu m}$\dotfill &Blackbody eclipse depth at 2.5$\mu$m (ppm)\dotfill &$1371^{+24}_{-23}$\\
~~~~$\delta_{S,5.0\mu m}$\dotfill &Blackbody eclipse depth at 5.0$\mu$m (ppm)\dotfill &$3422^{+29}_{-26}$\\
~~~~$\delta_{S,7.5\mu m}$\dotfill &Blackbody eclipse depth at 7.5$\mu$m (ppm)\dotfill &$4456^{+28}_{-24}$\\
~~~~$\rho_P$\dotfill &Density (cgs)\dotfill &$0.633\pm0.034$\\
~~~~$logg_P$\dotfill &Surface gravity \dotfill &$3.226^{+0.021}_{-0.023}$\\
~~~~$\Theta$\dotfill &Safronov Number \dotfill &$0.0467^{+0.0025}_{-0.0024}$\\
~~~~$\fave$\dotfill &Incident Flux (\fluxcgs)\dotfill &$1.666^{+0.056}_{-0.053}$\\
~~~~$T_P$\dotfill &Time of Periastron (\bjdtdb)\dotfill &$2454697.797525\pm0.000024$\\
~~~~$T_S$\dotfill &Time of eclipse (\bjdtdb)\dotfill &$2454697.128410\pm0.000024$\\
~~~~$T_A$\dotfill &Time of Ascending Node (\bjdtdb)\dotfill &$2454698.801199\pm0.000024$\\
~~~~$T_D$\dotfill &Time of Descending Node (\bjdtdb)\dotfill &$2454698.132083\pm0.000024$\\
~~~~$V_c/V_e$\dotfill & \dotfill &$1.00$\\
~~~~$M_P\sin i$\dotfill &Minimum mass (\mj)\dotfill &$1.197^{+0.071}_{-0.066}$\\
~~~~$M_P/M_*$\dotfill &Mass ratio \dotfill &$0.001304^{+0.000069}_{-0.000067}$\\
~~~~$d/R_*$\dotfill &Separation at mid transit \dotfill &$5.489^{+0.011}_{-0.019}$\\
~~~~$P_T$\dotfill &A priori non-grazing transit prob \dotfill &$0.15431^{+0.00049}_{-0.00031}$\\
~~~~$P_{T,G}$\dotfill &A priori transit prob \dotfill &$0.21006^{+0.00075}_{-0.00041}$\\
\smallskip\\\multicolumn{2}{l}{Wavelength Parameters:}&R&z'&TESS\smallskip\\
~~~~$u_{1}$\dotfill &linear limb-darkening coeff \dotfill &$0.421\pm0.015$&$0.300^{+0.012}_{-0.013}$&$0.328\pm0.016$\\
~~~~$u_{2}$\dotfill &quadratic limb-darkening coeff \dotfill &$0.238^{+0.021}_{-0.022}$&$0.262\pm0.023$&$0.224\pm0.025$\\
\smallskip\\\multicolumn{2}{l}{Telescope Parameters:}&CORALIE\smallskip\\
~~~~$\gamma_{\rm rel}$\dotfill &Relative RV Offset (m/s)\dotfill &$57732.6^{+7.4}_{-7.3}$\\
~~~~$\sigma_J$\dotfill &RV Jitter (m/s)\dotfill &$19.9^{+9.7}_{-7.4}$\\
~~~~$\sigma_J^2$\dotfill &RV Jitter Variance \dotfill &$400^{+480}_{-240}$\\
\smallskip\\\multicolumn{2}{l}{Transit Parameters:}&EulerCam UT 2007-09-25 (R)&FORS2 UT 2007-09-25 (z')&DFOSC UT 2008-08-19 (R)&MagIC UT 2008-08-19 (z')&DFOSC UT 2008-08-23 (R)&DFOSC UT 2008-09-23 (R)&DFOSC UT 2008-10-01 (R)&MagIC UT 2008-10-09 (z')&TESS UT 2018-07-01 (TESS)&TESS UT 2018-07-01 (TESS)&TESS UT 2018-07-01 (TESS)\smallskip\\
~~~~$\sigma^{2}$\dotfill &Added Variance \dotfill &$0.00000234^{+0.00000035}_{-0.00000031}$&$0.000000161^{+0.000000035}_{-0.000000030}$&$0.000000183^{+0.00000011}_{-0.000000092}$&$0.000000013^{+0.000000029}_{-0.000000026}$&$0.000000156^{+0.00000012}_{-0.000000100}$&$0.000000203^{+0.00000012}_{-0.000000096}$&$0.000000147^{+0.000000073}_{-0.000000063}$&$-0.000000303^{+0.000000020}_{-0.000000017}$&$-0.00000059\pm0.00000015$&$0.00000069\pm0.00000025$&$-0.00000057\pm0.00000016$\\
~~~~$F_0$\dotfill &Baseline flux \dotfill &$0.99974^{+0.00013}_{-0.00012}$&$1.000186^{+0.000043}_{-0.000041}$&$0.999856^{+0.000079}_{-0.000080}$&$0.999938\pm0.000035$&$0.999987^{+0.000083}_{-0.000081}$&$0.999568^{+0.000093}_{-0.000097}$&$1.000091^{+0.000071}_{-0.000070}$&$0.999927^{+0.000031}_{-0.000030}$&$1.000063\pm0.000040$&$1.000219^{+0.000053}_{-0.000056}$&$1.000101^{+0.000044}_{-0.000045}$\\
\enddata
\tablenotetext{}{See Table 3 in \citet{Eastman:2019} for a detailed description of all parameters}
\tablenotetext{1}{This value ignores the systematic error and is for reference only}
\tablenotetext{2}{The metallicity of the star at birth}
\tablenotetext{3}{Corresponds to static points in a star's evolutionary history. See \S2 in \citet{Dotter:2016}.}
\tablenotetext{4}{Time of conjunction is commonly reported as the "transit time"}
\tablenotetext{5}{Time of minimum projected separation is a more correct "transit time"}
\tablenotetext{6}{Optimal time of conjunction minimizes the covariance between $T_C$ and Period}
\tablenotetext{7}{Assumes no albedo and perfect redistribution}
\end{deluxetable*}

